A Constant Factor Approximation for Navigating Through Connected Obstacles in the Plane

Given two points s and t in the plane and a set of obstacles defined by closed curves, what is the minimum number of obstacles touched by a path connecting s and t? This is a fundamental and well-studied problem arising naturally in computational geometry, graph theory (under the names Min-Color Path and Minimum Label Path), wireless sensor networks (Barrier Resilience) and motion planning (Minimum Constraint Removal). It remains NP-hard even for very simple-shaped obstacles such as unit-length line segments. In this paper we give the first constant factor approximation algorithm for this problem, resolving an open problem of [Chan and Kirkpatrick, TCS, 2014] and [Bandyapadhyay et al., CGTA, 2020]. We also obtain a constant factor approximation for the Minimum Color Prize Collecting Steiner Forest where the goal is to connect multiple request pairs (s1, t1), . . . ,(sk, tk) while minimizing the number of obstacles touched by any (si, ti) path plus a fixed cost of wi for each pair (si, ti) left disconnected. This generalizes the classic Steiner Forest and Prize-Collecting Steiner Forest problems on planar graphs, for which intricate PTASes are known. In contrast, no PTAS is possible for Min-Color Path even on planar graphs since the problem is known to be APXhard [Eiben and Kanj, TALG, 2020]. Additionally, we show that generalizations of the problem to disconnected obstacles

==> Makefile <==
TEXSRC := document.tex
AUX := $(TEXSRC:.tex=.aux)
PDF := $(TEXSRC:.tex=.pdf)

all:
	pdflatex $(TEXSRC)
	-bibtex $(AUX)
	-pdflatex $(TEXSRC)
	-pdflatex $(TEXSRC)
	\rm -f *.aux *.log  *.blg *.out *.vtc *.brf 

clean:
	\rm -f *.aux *.log *.blg *.pdf *.vtc *.out *.brf




==> commands.tex <==

\long\def\cut#1{{}}
\def\cc{\mathcal{C}}
\def\cp{\mathcal{P}}
\def\ca{\mathcal{A}}
\def\cb{\mathcal{B}}
\def\cs{\mathcal{S}}
\def\cg{\mathcal{G}}
\def\cl{\mathcal{L}}
\def\cu{\mathcal{U}}
\def\rs{\mathcal{R}} %range space
%\def\opt{\textit{OPT}}
\newcommand{\np}{\textsf{NP}}
\def\eps{\epsilon}
\def\mathify#1{\ifmmode{#1}\else\mbox{$#1$}\fi} % guarantee math mode
\let\ensuremath=\mathify
\newcommand{\cd}{\mathcal{D}}
\newcommand{\co}{\mathcal{S}}
\newcommand{\cn}{\mathcal{N}}
\newcommand{\ce}{\mathcal{E}}
\newcommand{\cm}{\mathcal{M}}
\newcommand{\apx}{\textsf{APX}}
\def\seg#1{\ensuremath{\overline{#1}}}
\def\GA{G_{\mathcal A}}
\def\cost{\emph{cost}}
\def\weight{\emph{weight}}
%==== macros and packages =====
\usepackage{microtype}%if unwanted, comment out or use option "draft"
\usepackage{wrapfig}
\usepackage{yhmath}
\usepackage{xcolor}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{algorithm}

\newtheorem{observation}{Observation}[section]
\newtheorem{claim}{Claim}[section]

\RequirePackage{fix-cm}
%\smartqed  % flush right qed marks, e.g. at end of proof
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{color}
%\usepackage[nocompress]{cite}
\usepackage{wrapfig}
\usepackage{blindtext}
\allowdisplaybreaks

\usepackage{mdframed}
\usepackage{multirow}
\newcommand{\cv}{U}

\def\seg#1{\ensuremath{\overline{#1}}}
\def\GA{G_{\mathcal A}}
\def\cost{\emph{cost}}
\def\weight{\emph{weight}}

\def\opt{\textit{OPT}}

\def\ct{\mathcal{T}}
\def\ci{\mathcal{I}}
\def\cx{\mathcal{X}}
\def\cw{\mathcal{W}}
\def\cz{\mathcal{Z}}
\def\cf{\mathcal{F}}
\def\adj{\textit{adj}}
\def\mcp{\textsc{Min-Color Path}\xspace}
\def\dvrconj{\textsc{Dense vs Random}\xspace}
\def\lp{\textsc{Hitting-LP}\xspace}
\def\wt{w}
\def\rep{\textit{rep}}
\def\planarMCP{\textsc{Planar-Conn-MCP}\xspace}

\usepackage{enumitem,xparse}
\usepackage{soul}

\def\yellow#1{{\hl{#1}}}

